Discrete hypocoercive estimates for discontinuous Galerkin methods: application to the Vlasov-Poisson-Fokker-Planck system

We develop and analyze a class of structure-preserving discontinuous Galerkin schemes for the nonlinear Vlasov-Poisson-Fokker-Planck model, reformulated as a hyperbolic system through a Hermite expansion in the velocity variable. We discretize the Vlasov-Fokker-Planck equation with the discontinuous Galerkin method, while the Poisson equation is approximated with either a discontinuous Galerkin method or a Raviart-Thomas mixed finite element method. We prove the exponential relaxation to equilibrium for suitable initial data, uniformly with respect to the discretization parameters thanks to discrete hypocoercivity arguments. Moreover, we check that the resulting semi-discrete schemes preserve the physical invariants along with the L 2 variational structure of the linearized model. Numerical simulations verify the accuracy and the long-time behavior of the scheme.

==> elsback.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ACKNOWLEDGEMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Acknowledgments}

The first author acknowledges the financial support of the Graduate School of Xiamen University.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BIBLIOGRAPHY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \bibliographystyle{siamplain}
\bibliographystyle{elsarticle-num}
\bibliography{P2_VPFP_DGHS}



==> elsfront.tex <==
\begin{frontmatter}

    % Title, authors, and affiliations
    \title{On the long-time behavior of discontinuous Galerkin/Hermite spectral method for the Vlasov-Poisson-Fokker-Planck model}
    \author[1]{Yi Cai}
    \ead{yicaim@stu.xmu.edu.cn}

    \address[1]{School of Mathematical Sciences, Xiamen University, Xiamen, Fujian 361005, PR China}

    \author[2]{Francis Filbet\corref{correspondingauthor}}
    \address[2]{Institut de Math{\'e}matiques de Toulouse, Universit{\'e} Paul Sabatier, Toulouse 31062, France}
    \ead{francis.filbet@math.univ-toulouse.fr}

    \author[3]{Alain Blaustein}
    \ead{alain.blaustein@inria.fr}

    \address[3]{Centre Inria de l'Universit{\'e} de Lille, France}

    \author[4]{Tao Xiong}
    \ead{taoxiong@ustc.edu.cn}

    \address[4]{School of Mathematical Sciences, University of Science and Technology of China, Hefei, Anhui 230026, PR China}

    \cortext[correspondingauthor]{Corresponding author.}

    \begin{abstract} 
    We develop a class of discontinuous Galerkin (DG) schemes for the nonlinear Vlasov-Poisson-Fokker-Planck model, reformulated as a hyperbolic system through a Hermite expansion in the velocity variable. We discretize the Vlasov-Fokker-Planck equation by the DG method, while the Poisson equation is approximated by either a DG method or a Raviart-Thomas mixed finite element method. The resulting semi-discrete schemes preserve a discrete $L^2$ free energy estimate. Moreover, with an appropriate choice of numerical fluxes, we adapt hypocoercivity arguments to derive quantitative estimates on the exponential relaxation to discrete equilibrium for suitable initial data, uniformly with respect to the discretization parameters. Numerical simulation verifies the accuracy and long-time behavior of the scheme.
    \end{abstract}

    % Keywords
    \begin{keyword}
        Hermite spectral method \sep Discontinuous Galerkin method \sep Vlasov-Poisson-Fokker-Planck \sep Hypocoercive estimates
    \end{keyword}

\end{frontmatter}


